EC-Guide: A Comprehensive E-Commerce Guide for Instruction Tuning and Quantization

Large language models (LLMs) have attracted considerable attention in various fields for their cost-effective solutions to diverse challenges, especially with advancements in instruction tuning and quantization. E-commerce, with its complex tasks and extensive product-user interactions, presents a promising application area for LLMs. However, the domain-specific concepts and knowledge inherent in e-commerce pose significant challenges for adapting general LLMs. To address this issue, we developed EC-Guide \href{https://github.com/fzp0424/EC-Guide-KDDUP-2024}, a comprehensive e-commerce guide for instruction tuning and quantization of LLMs. We also heuristically integrated Chain-of-Thought (CoT) during inference to enhance arithmetic performance. Our approach achieved the 2nd place in Track 2 and 5th place in Track 5 at the Amazon KDD Cup'24 \href{https://www.aicrowd.com/challenges/amazon-kdd-cup-2024-multi-task-online-shopping-challenge-for-llms}. Additionally, our solution is model-agnostic, enabling effective scalability across larger systems.

==> Table/gpu.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[htbp]
\centering
\caption{GPU USAGE}
\label{tab:gpu}
\resizebox{.75\linewidth}{!}{%
\begin{tabular}{lccl} 
\toprule
\textbf{\textbf{\textbf{\textbf{Model}}}} & \textbf{PTQ}     & \begin{tabular}[c]{@{}c@{}}\textbf{Loading Model Weights }\\\textbf{(4 GPU Average)}\end{tabular} & \textbf{dtype}            \\ 
\midrule
Qwen2-7B                                  & \textbackslash{} & 3.55 GB                                                                                           & \multirow{6}{*}{float16}  \\
GLM-4-9B                                  & \textbackslash{} & 4.45GB                                                                                            &                           \\
Qwen1.5-14B                               & \textbackslash{} & 6.65GB                                                                                            &                           \\
\multirow{3}{*}{Yi-1.5-34B}                   & INT4             & 4.55GB                                                                                            &                           \\
                                          & INT8             & 8.47GB                                                                                            &                           \\
                                          & \textbackslash{} & 16.04GB                                                                                           &                           \\
\bottomrule
\end{tabular}%
}
\end{table}
